Learning Sparse Mixture of Experts for Visual Question Answering

There has been a rapid progress in the task of Visual Question Answering with improved model architectures. Unfortunately, these models are usually computationally intensive due to their sheer size which poses a serious challenge for deployment. We aim to tackle this issue for the specific task of Visual Question Answering (VQA). A Convolutional Neural Network (CNN) is an integral part of the visual processing pipeline of a VQA model (assuming the CNN is trained along with entire VQA model). In this project, we propose an efficient and modular neural architecture for the VQA task with focus on the CNN module. Our experiments demonstrate that a sparsely activated CNN based VQA model achieves comparable performance to a standard CNN based VQA model architecture.

==> Visual QA workshop submission arXiv/conv_clevr.tex <==
\newcommand{\blockx}[3]{\multirow{3}{*}{
\(\left[
\begin{array}{l}
\text{1$\times$1, #2}\\
[-.1em] \text{3$\times$3, #2, $C$=12}\\
[-.1em] \text{1$\times$1, #1}\\
\end{array}\right]\)$\times$#3}
}

% \newcolumntype{x}[1]{>\centering p{#1pt}}
% \newcommand{\ft}[1]{\fontsize{#1pt}{1em}\selectfont}
\renewcommand\arraystretch{1.25}
\setlength{\tabcolsep}{1.2pt}
\begin{table}[t]
\begin{center}
\footnotesize
% \begin{tabular}{c|c|x{80}}
\begin{tabular}{c|c|c}
\hline
stage & output & Description \\
\hline
conv1 & \ft{7} 64$\times$64 & 3$\times$3, 64, stride 2 \\
\hline
\multirow{4}{*}{conv2} & \multirow{4}{*}{\ft{7} 32$\times$32} & 3$\times$3 max pool, stride 2 \\\cline{3-3}
  &  & \blockx{48}{48}{1}\\
  &  & \\
  &  & \\
\hline
\multirow{3}{*}{conv3} &  \multirow{3}{*}{\ft{7} 16$\times$16} 
  &  \blockx{48}{48}{1}\\
  &  & \\
  &  & \\
\hline
\multirow{3}{*}{conv4} & \multirow{3}{*}{\ft{7} 8$\times$8} 
  &  \blockx{48}{48}{1}\\
  &  & \\
  &  & \\
\hline
conv5 & {\ft{7} 8$\times$8} & \specialcell{$1\times1$ conv. layer\\with 24 o/p channels}\\
\hline
\end{tabular}
\end{center}
%\vspace{1em}
\caption{Modular CNN for Relational Networks Model}
\label{tab:cnn_clevr}
\vspace{-.5em}
\end{table}

==> Visual QA workshop submission arXiv/conv_combined.tex <==
\newcommand{\blockxvqa}[3]{\multirow{3}{*}{
\(\left[
\begin{array}{l}
\text{1$\times$1, #2}\\
[-.1em] \text{3$\times$3, #2, $C$=32}\\
[-.1em] \text{1$\times$1, #1}\\
\end{array}\right]\)$\times$#3}
}

\newcommand{\blockx}[3]{\multirow{3}{*}{
\(\left[
\begin{array}{l}
\text{1$\times$1, #2}\\
[-.1em] \text{3$\times$3, #2, $C$=12}\\
[-.1em] \text{1$\times$1, #1}\\
\end{array}\right]\)$\times$#3}
}

% \newcolumntype{x}[1]{>\centering p{#1pt}}
% \newcommand{\ft}[1]{\fontsize{#1pt}{1em}\selectfont}
\renewcommand\arraystretch{1.25}
\setlength{\tabcolsep}{1.2pt}
\begin{table}[t]
\parbox{.45\linewidth}{
\centering
\footnotesize
\begin{tabular}{c|c|c}
\hline
 stage & output & Description \\
\hline
conv1 & \ft{7} 112$\times$112 & 7$\times$7, 64, stride 2 \\
\hline
\multirow{4}{*}{conv2} & \multirow{4}{*}{\ft{7} 56$\times$56} & 3$\times$3 max pool, stride 2 \\\cline{3-3}
  &  &  \blockxvqa{256}{128}{3}\\
  &  & \\
  &  & \\
\hline
\multirow{3}{*}{conv3} &  \multirow{3}{*}{\ft{7} 28$\times$28} 
  & \blockxvqa{512}{256}{4}\\
  &  & \\
  &  & \\
\hline
\multirow{3}{*}{conv4} & \multirow{3}{*}{\ft{7} 14$\times$14} 
  & \blockxvqa{1024}{512}{23}\\
  &  & \\
  &  & \\
\hline
\multirow{3}{*}{conv5} & \multirow{3}{*}{\ft{7} 7$\times$7} 
& \blockxvqa{2048}{1024}{3}\\
  &  & \\
  &  & \\
\hline
\end{tabular}
%\vspace{1em}
\caption{Modular CNN for VQA v2 model}
\label{tab:cnn_vqa}
% \vspace{-.5em}
% \end{table}
}
% \newcolumntype{x}[1]{>\centering p{#1pt}}
% \newcommand{\ft}[1]{\fontsize{#1pt}{1em}\selectfont}
\hfill
\parbox{.45\linewidth}{
\centering
% \renewcommand\arraystretch{1.25}
% \setlength{\tabcolsep}{1.2pt}
% \begin{table}[t]
\footnotesize
% \begin{tabular}{c|c|x{80}}
\begin{tabular}{c|c|c}
\hline
stage & output & Description \\
\hline
conv1 & \ft{7} 64$\times$64 & 3$\times$3, 64, stride 2 \\
\hline
\multirow{4}{*}{conv2} & \multirow{4}{*}{\ft{7} 32$\times$32} & 3$\times$3 max pool, stride 2 \\\cline{3-3}
  &  & \blockx{48}{48}{1}\\
  &  & \\
  &  & \\
\hline
\multirow{3}{*}{conv3} &  \multirow{3}{*}{\ft{7} 16$\times$16} 
  &  \blockx{48}{48}{1}\\
  &  & \\
  &  & \\
\hline
\multirow{3}{*}{conv4} & \multirow{3}{*}{\ft{7} 8$\times$8} 
  &  \blockx{48}{48}{1}\\
  &  & \\
  &  & \\
\hline
conv5 & {\ft{7} 8$\times$8} & \specialcell{$1\times1$ conv. layer\\with 24 o/p channels}\\
\hline
\end{tabular}
\caption{Modular CNN for Relational Networks Model}
\label{tab:cnn_clevr}
% \vspace{-.5em}
}
\end{table}

==> Visual QA workshop submission arXiv/conv_vqa.tex <==
\newcommand{\blockxvqa}[3]{\multirow{3}{*}{
\(\left[
\begin{array}{l}
\text{1$\times$1, #2}\\
[-.1em] \text{3$\times$3, #2, $C$=32}\\
[-.1em] \text{1$\times$1, #1}\\
\end{array}\right]\)$\times$#3}
}

% \newcolumntype{x}[1]{>\centering p{#1pt}}
% \newcommand{\ft}[1]{\fontsize{#1pt}{1em}\selectfont}
\renewcommand\arraystretch{1.25}
\setlength{\tabcolsep}{1.2pt}
\begin{table}[t]
\begin{center}
\footnotesize
\begin{tabular}{c|c|c}
\hline
 stage & output & Description \\
\hline
conv1 & \ft{7} 112$\times$112 & 7$\times$7, 64, stride 2 \\
\hline
\multirow{4}{*}{conv2} & \multirow{4}{*}{\ft{7} 56$\times$56} & 3$\times$3 max pool, stride 2 \\\cline{3-3}
  &  &  \blockxvqa{256}{128}{3}\\
  &  & \\
  &  & \\
\hline
\multirow{3}{*}{conv3} &  \multirow{3}{*}{\ft{7} 28$\times$28} 
  & \blockxvqa{512}{256}{4}\\
  &  & \\
  &  & \\
\hline
\multirow{3}{*}{conv4} & \multirow{3}{*}{\ft{7} 14$\times$14} 
  & \blockxvqa{1024}{512}{23}\\
  &  & \\
  &  & \\
\hline
\multirow{3}{*}{conv5} & \multirow{3}{*}{\ft{7} 7$\times$7} 
& \blockxvqa{2048}{1024}{3}\\
  &  & \\
  &  & \\
\hline
\end{tabular}
\end{center}
%\vspace{1em}
\caption{Modular CNN for VQA v2 model}
\label{tab:cnn_vqa}
\vspace{-.5em}
\end{table}

==> Visual QA workshop submission arXiv/related_work.tex <==
% Background
\section{Related Work}
% \large
% ResNeXt \cite{xie2017aggregated} introduces cardinality as a new dimension in convolutional networks, apart from width and depth. The paper shows that increasing the cardinality is a more effective way to increase capacity for better performance. Squeeze-and-Excitation Networks \cite{hu2017squeeze} proposes attention on channel-wise features, and improves the state of the art in ILSVRC. Using a sparse combination of expert networks has been explored in \cite{shazeer2017outrageously} for language modelling tasks. Use of mixture-of-experts formulation for sparsifying channel features has been explored in \cite{wang2018deep}. A modularized version of ResNet is proposed in \cite{jo2018modularity} for visual reasoning tasks.
\textbf{Mixture of Experts} Mixture of Experts \cite{jacobs1991adaptive} is a formulation in machine learning which employs the divide-and-conquer principle to solve a complex problem by dividing the neural network into several expert networks. In the Mixture of MLP Experts (MME) method \cite{waterhouse1998classification, nguyen2006cooperative, ebrahimpour2008view}, a gating network is used to assign weights to the outputs of the corresponding expert networks. The gating network is an MLP followed by softmax operator. The final output of the ensemble is a weighted sum of outputs of each of the individual expert networks.
% a gating network is used to assign a weight $g_i$ to the output of the corresponding expert network. The final output of the ensemble is a weighted sum of outputs of each of the individual expert networks, 
% $$ \bm{O} = \sum_{i=1}^N \bm{o}_i g_i$$
% where, we have $N$ experts and $\bm{o}_i$ denotes the output of the $i^{th}$ expert.
\cite{jo2018modularity} uses a mixture of experts for visual reasoning tasks in which each expert is a stack of residual blocks.

\textbf{Conditional Computation} Conditional Computation is the technique of activating only a sub-portion of the neural network depending on the inputs. For instance, if a visual question answering system has to count the number of a specified object \textit{vs} if it has to tell the color of an object, the specific features needed to give the correct answer in either case are different. Hence, there is a potential to reduce the amount of computation the network has to perform in each case, which can be especially useful to train large deep networks efficiently. The use of stochastic neurons with binary outputs to selectively turn-off experts in a neural network has been explored in \cite{bengio2013estimating}. \cite{davis2013low} uses a low-rank approximation of weight matrix of MLP to compute the sign of pre-nonlinearity activations. In case of ReLU activation function, it is then used to optimize the matrix multiplication for the MLP layer. \cite{bengio2015conditional} uses Policy gradient to sparsely activate units in feed-forward neural networks by relying on conditional computation. \cite{shazeer2017outrageously} proposes Sparsely-Gated Mixture-of-Experts layer (MoE) which uses conditional computation to train huge capacity models on low computational budget for language modeling and machine translation tasks. It makes use of noisy top-$K$ mechanism in which a random noise is added to gating weights and then top-$K$ weights are selected. Another line of work makes use of conditional computation in VQA setting. DPPNet \cite{noh2015dppnet} makes use of a dynamic parameter layer (fully-connected) conditioned on the question representation for VQA. ABC-CNN \cite{Chen2015ABCCNNAA} predicts convolutional kernel weights using an MLP which takes question representation as input. Here, the advantage is that the question conditioned convolutional kernels can filter out unrelated image regions in the visual processing pipeline itself.

\textbf{Computationally efficient CNNs} \cite{huang2017multi} proposes Multi-Scale Dense Convolutional Networks (MSDNet) to address two key issues in (i) budgeted classification- distribute the computation budget unevenly across easy and hard examples, (ii) anytime prediction: the network can output the prediction result at at any layer depending on the computation budget without significant loss in accuracy. The optimization of computational complexity of CNNs at inference-time has been studied in \cite{bolukbasi2017adaptive} in which an adaptive early-exit strategy is learned to by-pass some of the network's layers in order to save computations. MobileNet \cite{howard2017mobilenets} uses depth-wise separable convolutions to build light weight CNNs for deployment on mobile devices. 

\textbf{CNN architectures} The invention of Convolutional Neural Networks (CNNs) has led to a remarkable improvement in performance for many computer vision tasks \cite{krizhevsky2012imagenet, long2015fully, ren2015faster}. In recent years, there has been a spate of different CNN architectures with changes to depth \cite{simonyan2014very}, topology \cite{he2016deep, szegedy2015going}, etc. The use of \textit{split-transform-merge} strategy for designing convolutional blocks (which can be stacked to form the complete network) has shown promise for achieving top performance with a lesser computational complexity \cite{szegedy2015going, szegedy2017inception, szegedy2016rethinking, xie2017aggregated}. The ResNeXt \cite{xie2017aggregated} CNN model proposes cardinality (size of set of transformations in a convolutional block) as another dimension apart from depth and width to investigate, for improving the performance of convolutional neural networks. Squeeze-and-Excitation Networks \cite{hu2017squeeze} proposes channel-wise attention in a convolutional block and helped improve the state of art in ILSVRC 2017 classification competition.

\textbf{Grouped Convolution} In grouped convolution, each filter convolves only with the input feature maps in its group. The use of grouped convolutions was first done in AlexNet \cite{krizhevsky2012imagenet} for training a large network on 2 GPUs. A recently proposed CNN architecture named CondenseNet \cite{huang2018condensenet} makes use of learned grouped convolutions to minimise superfluous feature-reuse and achieve computational efficiency.  



==> conv_combined.tex <==
\newcommand{\blockxvqa}[3]{\multirow{3}{*}{
\(\left[
\begin{array}{l}
\text{1$\times$1, #2}\\
[-.1em] \text{3$\times$3, #2, $C$=32}\\
[-.1em] \text{1$\times$1, #1}\\
\end{array}\right]\)$\times$#3}
}

\newcommand{\blockx}[3]{\multirow{3}{*}{
\(\left[
\begin{array}{l}
\text{1$\times$1, #2}\\
[-.1em] \text{3$\times$3, #2, $C$=12}\\
[-.1em] \text{1$\times$1, #1}\\
\end{array}\right]\)$\times$#3}
}

% \newcolumntype{x}[1]{>\centering p{#1pt}}
% \newcommand{\ft}[1]{\fontsize{#1pt}{1em}\selectfont}
\renewcommand\arraystretch{1.25}
\setlength{\tabcolsep}{1.2pt}
\begin{table}[t]
\parbox{.45\linewidth}{
\centering
\footnotesize
\begin{tabular}{c|c|c}
\hline
 stage & output & Description \\
\hline
conv1 & \ft{7} 112$\times$112 & 7$\times$7, 64, stride 2 \\
\hline
\multirow{4}{*}{conv2} & \multirow{4}{*}{\ft{7} 56$\times$56} & 3$\times$3 max pool, stride 2 \\\cline{3-3}
  &  &  \blockxvqa{256}{128}{3}\\
  &  & \\
  &  & \\
\hline
\multirow{3}{*}{conv3} &  \multirow{3}{*}{\ft{7} 28$\times$28} 
  & \blockxvqa{512}{256}{4}\\
  &  & \\
  &  & \\
\hline
\multirow{3}{*}{conv4} & \multirow{3}{*}{\ft{7} 14$\times$14} 
  & \blockxvqa{1024}{512}{23}\\
  &  & \\
  &  & \\
\hline
\multirow{3}{*}{conv5} & \multirow{3}{*}{\ft{7} 7$\times$7} 
& \blockxvqa{2048}{1024}{3}\\
  &  & \\
  &  & \\
\hline
\end{tabular}
%\vspace{1em}
\caption{Modular CNN for VQA v2 model}
\label{tab:cnn_vqa}
% \vspace{-.5em}
% \end{table}
}
% \newcolumntype{x}[1]{>\centering p{#1pt}}
% \newcommand{\ft}[1]{\fontsize{#1pt}{1em}\selectfont}
\hfill
\parbox{.45\linewidth}{
\centering
% \renewcommand\arraystretch{1.25}
% \setlength{\tabcolsep}{1.2pt}
% \begin{table}[t]
\footnotesize
% \begin{tabular}{c|c|x{80}}
\begin{tabular}{c|c|c}
\hline
stage & output & Description \\
\hline
conv1 & \ft{7} 64$\times$64 & 3$\times$3, 64, stride 2 \\
\hline
\multirow{4}{*}{conv2} & \multirow{4}{*}{\ft{7} 32$\times$32} & 3$\times$3 max pool, stride 2 \\\cline{3-3}
  &  & \blockx{48}{48}{1}\\
  &  & \\
  &  & \\
\hline
\multirow{3}{*}{conv3} &  \multirow{3}{*}{\ft{7} 16$\times$16} 
  &  \blockx{48}{48}{1}\\
  &  & \\
  &  & \\
\hline
\multirow{3}{*}{conv4} & \multirow{3}{*}{\ft{7} 8$\times$8} 
  &  \blockx{48}{48}{1}\\
  &  & \\
  &  & \\
\hline
conv5 & {\ft{7} 8$\times$8} & \specialcell{$1\times1$ conv. layer\\with 24 o/p channels}\\
\hline
\end{tabular}
\caption{Modular CNN for Relational Networks Model}
\label{tab:cnn_clevr}
% \vspace{-.5em}
}
\end{table}
